Cheaters in the Steam Community Gaming Social Network

Online gaming is a multi-billion dollar industry that entertains a large, global population. One unfortunate phenomenon, however, poisons the competition and the fun: cheating. The costs of cheating span from industry-supported expenditures to detect and limit cheating, to victims' monetary losses due to cyber crime. This paper studies cheaters in the Steam Community, an online social network built on top of the world's dominant digital game delivery platform. We collected information about more than 12 million gamers connected in a global social network, of which more than 700 thousand have their profiles flagged as cheaters. We also collected in-game interaction data of over 10 thousand players from a popular multiplayer gaming server. We show that cheaters are well embedded in the social and interaction networks: their network position is largely undistinguishable from that of fair players. We observe that the cheating behavior appears to spread through a social mechanism: the presence and the number of cheater friends of a fair player is correlated with the likelihood of her becoming a cheater in the future. Also, we observe that there is a social penalty involved with being labeled as a cheater: cheaters are likely to switch to more restrictive privacy settings once they are tagged and they lose more friends than fair players. Finally, we observe that the number of cheaters is not correlated with the geographical, real-world population density, or with the local popularity of the Steam Community. This analysis can ultimately inform the design of mechanisms to deal with anti-social behavior (e.g., spamming, automated collection of data) in generic online social networks.

==> sections/general-stats.tex <==
\section{Cheaters in the Community}
\label{sec:eval}

 While this paper focuses mainly on aspects of social network
 analysis to understand the position of cheaters in the network, we
 also look at some general behavioral characteristics independent of
 the network structure. In particular, we are interested in
 understanding patterns that might differentiate cheaters from the
 overall \emph{Steam Community} population in terms of game play
 time, games owned, and geographical distribution.  



\subsection{Gameplay Statistics}
\label{sec:gameplay-stats}
  
The hours played in the two weeks prior to the crawl for all users and
for cheaters is plotted as a CCDF in
Figure~\ref{fig:hours_played_ccdf}.
We observe that cheaters play less time
than the general population.
%, but this difference begins to converge as the number of hours played increases.  
We also note that a few users appear as having played
for more hours in a two week period than there are hours in
that interval: there are 95 users with over 336 hours played (3 of
which are cheaters).   The maximum hours played was 1285.8 (over two
weeks), and   coincidentally, the honor of most hours played belongs
to a cheater.
We believe these impossible amounts of hours played are attributable to either account sharing, where multiple players accumulated a large amount of play time attached to the same account, or a reporting error.
%Of these 95 players, 48 had a location set.
%Of those 48, 24 were from the United States, 5 from the Nordic countries of Sweden, Norway, Finland, and Denmark, 3 from Germany, 3 from Russia, 2 from Poland, 2 from Canada, and 1 player from 9 other countries.


%\begin{figure}[th]
%    \centering
%\includegraphics[scale=1.0]{figures/hoursplayed_numusers_ccdf_10193-test.pdf}
%    \caption{CCDF for the
%      number of hours played in the two weeks prior to the crawl.} 
%    \label{fig:hours_played_ccdf}
%   \end{figure}  
   

We find that the number of hours played increases with the number of
games a user owns up until around $80$ games owned for the cheaters and $200$ for the whole community (Figure~\ref{fig:games_owned_hours_played}).
%at which point it flattens out.
This is a somewhat
counter-intuitive result: there is limited time in a
two-week span, so one would imagine more games owned translates into
less time per game or favoring some games over the others. However,
that initial intuition disregards the question of causality.
I.e., does the acquisition of a new game result in an increase in hours played, or do users that play many hours seek out and purchase new games to stave off boredom?
%We do in fact see these two classes of users.
%Those with less than about 15 games acquire new games and in turn play more hours, while a new game acquisition for those that already have 15 games does not result in significantly more play time.

Finally, we note that no discernible pattern exists for the 95,890 users that own more than about $100$--$200$ games.
One possible explanation for this breakdown has to do with how games go on sale.
There are weekly sales on \emph{Steam}, and at least two seasonal ``mega-sales'' where users can purchase games at very steep discounts (in excess of 75\% off).
     Often times, especially for the seasonal sales, games are at a deep discount when purchased in \emph{packs}.
   %  E.g., when purchased together, 5 games might cost \$10.00 in total, but cost \$2.50 a piece when purchased individually.
     Thus, we suspect there are a significant number of users that
     might have purchased game packs offered at deep discount, sometimes
     without ever intending to play several of the games
     included in the pack.

    
Interestingly, cheaters own fewer games per hours played than the
community as a whole and tend to reach their saturation point, with
respect to game ownerships, sooner. This could be an effect of the
non-transferability of game licenses and the permanency of a VAC ban: the average cheater might be caught
and create new accounts before she has the opportunity to amass a
large collection of games.
  
           % 
           % It could be indicative of free riding behavior from the stand point of 1) other players and 2) game developers.
           % Cheaters free ride off of the community donated resources of other players, and, in general, make playing games not fun.
           % Related to this, they are a drain on game developers as 
           % 
           % 
           % They also do not seem to support 
           % 
           % 
           % Further contributing to the underlying business model type b while still playing
 
\begin{figure}[th]
\centering
	\subfigure[]{
		\includegraphics[width=1.75in]{figures/hoursplayed_numusers_ccdf_10193-test.pdf}
    		\label{fig:hours_played_ccdf}
		}
	\subfigure[]{
		\includegraphics[width=1.75in]{figures/gamesowned_hoursplayed_avg_10193-test.pdf}	
		\label{fig:games_owned_hours_played}
		}
\caption{
(a) CCDF for the number of hours played in the two weeks prior to the crawl.
(b) The average number of hours played across all games by all users owning the same number of games, vs. number of games.}
\end{figure}

 
%     \begin{figure}[th]
%      \centering
% \includegraphics[scale=1.0]{figures/gamesowned_hoursplayed_avg_10193-test.pdf}
%      \caption{The average number of hours played
%        across all games by all users owning the same number of
%        games, vs. number of games.} 
%      \label{fig:games_owned_hours_played}
%     \end{figure}
     
   
     % We observe a linearly increasing relationship\footnote{IS THIS TRUE? IS IT WITH RESPECT TO THE LOG OF THE NUMBER OF GAMES OWNED?!?} between the number of hours a user plays and the number of games owned by that user up until around 100 games owned, at which point no real pattern can be seen.

     % By looking at the number of hours played as a function of the number of games a user owns for all users as well as cheaters only we see an increasing relations 
      
\subsection{Group Membership}

Group membership was determined by querying the crawled users group memberships.
I.e., the list of groups, as well as each group's members were inferred from information in user profiles.
Because of this there are two caveats: 1)~users with private profiles are not included in the data set and 2)~there are likely some group members that were not discovered via our crawl.
Both of these mean that our results might differ slightly from ground truth, however, they should be pretty close.
We discovered over 5 million users that were members of at least one of over 1 million groups.
Table~\ref{tbl:groups} contains details of this data set.


\begin{table}
\begin{center}
\begin{tabular}{| l | r |}
  \hline
  Users in at least one group & 5,302,072 \\
  \hline
  Groups & 1,487,551 \\
  \hline
  Groups with at least 2 members & 1,160,793 \\
  \hline
  Average group members & 20.9 \\
  \hline
  Average groups per user & 3.56 \\
  \hline
  Maximum groups per user & 2,380 \\
  \hline
\end{tabular}
\end{center}
\caption{Details for groups data set inferred from the Steam Community profiles data set.}
\label{tbl:groups}
\end{table}

% \begin{figure}[th]
%  \centering \includegraphics[scale=1.0]{figures/groups/users_per_group_groups_per_user.pdf}
%   \caption{CDF of the members per group and groups per user.}
%   \label{fig:users_per_group_groups_per_user_cdf}
% \end{figure}

%\begin{figure}[th]
% \centering \includegraphics[scale=1.0]{figures/groups/num_groups_per_user_cheater_vs_noncheater_cdf.pdf}
%  \caption{CDF of the number of groups per user for cheaters and non-cheaters.}
%  \label{fig:num_groups_per_user_cheater_vs_noncheater_cdf}
%\end{figure}


About 90\% of the over 1 million groups had less than 31 members, and only 1\% had more than 150 members.
These membership numbers are similar to the observed sizes of guilds in World of Warcraft where the 90th percentile of the membership distribution was found to be 35~\cite{life_and_death_of_guild}.
Of the over 5 million users in at least one group, about 35\% were in one, and only one, group with 80\% of users were in less than 10 groups.
Somewhat surprisingly, cheaters tend to be members of more groups than non-cheaters, as seen in Figure~\ref{fig:num_groups_per_user_cheater_vs_noncheater_cdf}.


%\begin{figure}[th]
%  \centering
% \includegraphics[scale=1.0]{figures/groups/fraction_cheaters_per_group_min_2_members.pdf}
% \caption{Fraction of group members that are cheaters for groups with a minimum of 2 members.}
% \label{fig:fraction_cheaters_per_group_min_2_members}
%\end{figure}

\begin{figure}[th]
\centering
	\subfigure[]{
		\includegraphics[width=1.75in]{figures/groups/num_groups_per_user_cheater_vs_noncheater_cdf.pdf}
    		\label{fig:num_groups_per_user_cheater_vs_noncheater_cdf}
		}
	\subfigure[]{
		\includegraphics[width=1.75in]{figures/groups/fraction_cheaters_per_group_min_2_members.pdf}	
		\label{fig:fraction_cheaters_per_group_min_2_members}
		}
\caption{
(a) CDF of the number of groups per user for cheaters and non-cheaters.
(b) Fraction of group members that are cheaters for groups with a minimum of 2 members.}
\end{figure}


We next examined how cheaters and non-cheaters are represented in the group membership rolls.
We began by discarding groups with less than two members as at least two members are required for a social relationship to exist.
Of the remaining groups, we plot the fraction of members that are cheaters as a CDF in Figure~\ref{fig:fraction_cheaters_per_group_min_2_members}.
Our first observation is that cheaters are not evenly distributed in groups.
In fact, we note that in approximately 10\% of groups non-cheaters are a minority.
         

\subsection{Geographic Distribution}
    \ignore{ 
     
   \begin{figure*}[t]
        \centering
        \subfigure[User Locations]{
       \includegraphics[scale=1]{figures/user_loc.png}
       \label{fig:user_pop}
        }
        \subfigure[Cheater Locations]{
        \includegraphics[scale=1]{figures/cheater_loc.png}
        \label{fig:cheater_pop}
        }
        \label{fig:population}
        \caption{Percentile ranked geographic populations of users and cheaters in Steam Community. Populations are colored from red (top 1\%) to blue (bottom 99\%).}
       \end{figure*}
}

\begin{figure}[th]
 \centering
\includegraphics[scale=1.0]{figures/pop_countries_bar_stack.pdf}
 \caption{User and cheater populations per country normalized to real world population.} %The countries are listed on the x-axis by decreasing real world population.}
 \label{fig:pop_countries_bar_stack}
\end{figure}

We found that
user population on \emph{Steam Community} does not follow real-world
geographic population and that cheaters are not uniformly
distributed.  %Figure~\ref{fig:user_pop} indicates that some locations
%are over represented in the \emph{Steam Community} when considering their
%real world populations.
Figure~\ref{fig:pop_countries_bar_stack} shows \emph{Steam Community} populations for the twelve countries comprising the top ten user populations and the top ten cheater populations.
The countries are arranged along the x-axis in decreasing order of their real-world populations, and the number of \emph{Steam Community} non-cheaters and cheaters per country are normalized to the real-world population of said country.
There are about 1 million user accounts with a declared location in the United States, corresponding to around 0.33\% of the real population of the US, while there are approximately 445 thousand users in the Nordic European countries of Sweden, Denmark, Finland, and Norway, corresponding to around 1.7\% of these countries' real world populations.
Cheaters are vastly overrepresented in some
locations: for example, there are about 55,000 cheaters in the Nordic 
European countries (12.4\% of the playing population of the region),
while there are about 39,000 cheaters (3.9\%) in the US.
In particular, we found enough profiles to account for nearly 2.5\% of Denmark's 5.5$M$ residents, and cheaters account for nearly 0.5\% of the real-world population.

% Again we note that neither \emph{Steam Community} users nor cheaters are uniformly distributed with respect to real world populations.


% Figure~\ref{fig:degree_distribution} shows the degree distributions of the networks we extracted from Steam Community.
% In Figure~\ref{fig:degree_distribution_full} we can see an expected power law distribution with a quick fall off around $k = 250$.
% Unlike~\cite{Chun:2008wl}, we do not observe a two step distribution.
% This can be attributed to a hard upper limit of 250 friends imposed by Steam Community.

% Interestingly, we \emph{do} see some users with more than 250 friends.
% The maximum number of friends seen was 393 and belongs to a member of $V_{c}$; i.e., a cheater.
% We manually examined the profile of this account and confirmed a friends list of over 390 users.
% Further, we observed this number \emph{increasing} over several weeks while other anomalous friends lists of more than 250 users seemed to get trimmed upon manual examination.



